Fast algorithms for handling diagonal constraints in timed automata

A popular method for solving reachability in timed automata proceeds by enumerating reachable sets of valuations represented as zones. A na\"ive enumeration of zones does not terminate. Various termination mechanisms have been studied over the years. Coming up with efficient termination mechanisms has been remarkably more challenging when the automaton has diagonal constraints in guards. In this paper, we propose a new termination mechanism for timed automata with diagonal constraints based on a new simulation relation between zones. Experiments with an implementation of this simulation show significant gains over existing methods.

==> algorithms.tex <==
\section{Algorithms}

\noindent \textbf{Simulation using $\lug$.} The input to the algorithm
is a timed automaton $\Aa$. We assume that to each state $q$, a set of
guards $\Gg(q)$ is associated, satisfying the properties given in the
previous section. The algorithm maintains two lists, Passed and
Waiting. The initial zone $Z_0$ is is added to the Waiting list.
Wlog.\ we assume that $q_0$ is not accepting.  The algorithm
repeatedly performs the following steps:
\begin{description}
\item[Step 1.] If Waiting is empty, then return ``$\Aa$ has no
  accepting run''; else pick (and remove) a node $(q, Z)$ from
  Waiting.
\item[Step 2.] For each successor $(q, Z) \tto (q_1, Z_1)$ such that
  $Z_1 \neq \emptyset$ perform the following operations: if $q_1$ is
  accepting, return ``$\Aa$ has an accepting run''; else check if
  there exists a node $(q_1, Z_1')$ in Passed or Waiting s.t.
  $Z_1 \lugone Z_1'$: if yes, ignore the node $(q_1, Z_1)$, otherwise
  add $(q_1, Z_1)$ to Waiting.
\item[Step 3.] Add $(q, Z)$ to Passed and proceed to Step 1.
\end{description}

\noindent \textbf{Dynamically detecting relevant diagonal
  constraints.} The input to the algorithm is a timed automaton
$\Aa$. We want to associate a set of guards $\Gg$ at each node
$(q, Z)$ that will be computed, dynamically as and when more nodes are
discovered. We assume that initially $\Gg(q, Z)$ is the set of all
diagonal-free guards of $\Gg(q)$ computed statically as before. We are
only computing the relevant diagonal guards dynamically. The algorithm
maintains three lists: Passed, Waiting and Covered. The initial zone
$n_0:= (q_0,Z_0)$ is is added to the Waiting list, with $\Gg(n_0)$
being the diagonal-free guards of $\Gg(q_0)$.  Wlog.\ we assume that
$q_0$ is not accepting.  The algorithm repeatedly performs the
following steps:
\begin{description}
\item[Step 1.] If Waiting is empty:
  \begin{itemize}
  \item for all nodes $(q, Z)$ in Covered list: check if $Z \lug Z'$
    where $(q, Z')$ is the covering node, and $\Gg$ is the current set
    of guards at $(q, Z')$; if not covered, add $(q, Z)$ to Waiting
  \item if Waiting is still empty after the previous step, then return
    ``$\Aa$ has no accepting run''; else pick (and remove) a node
    $(q, Z)$ from Waiting.
  \end{itemize}
\item[Step 2.] For each successor $(q, Z) \tto (q_1, Z_1)$:
  \begin{itemize}
  \item if $Z_1 \neq \emptyset$ perform the following operations: if
    $q_1$ is accepting, return ``$\Aa$ has an accepting run''; else
    check if there exists a node $(q_1, Z_1')$ in Passed or Waiting
    s.t.  $Z_1 \lugone Z_1'$: if yes, add $(q_1, Z_1)$ to Covered,
    otherwise add $(q_1, Z_1)$ to Waiting;
  \item if $Z_1 = \emptyset$, perform a backward propagation to detect
    relevant diagonals (procedure explained below)
  \end{itemize}
\item[Step 3.] Add $(q, Z)$ to Passed and proceed to Step 1.
\end{description}

\noindent \textbf{Propagation operation.} The propagate operation
takes as arguments a transition $(q, Z) \xra[R]{g} (q_1, Z_1)$, and a
set of guards $\Gg_1$ at the target node $(q_1, Z_1)$. The function
computes a new set of guards that need to be added to $(q, Z)$.
\begin{itemize}
\item if $g$ is a diagonal constraint and
  $Z \not \sqsubseteq_{\scriptscriptstyle {\Gg_1}} Z \cap g$, then add
  all diagonal constraints of $\Gg_1$ and $g$ to the set of guards at
  $Z$; else add only the diagonal constraints of $\Gg_1$ to
  $\Gg((q, Z))$
\item if the above step changed the set of guards at $(q, Z)$ call the
  propagate function with respect to every incoming edge at $(q, Z)$
  (including covering edges);
  otherwise stop the propagation.
\end{itemize}

The aim of the above algorithm is to compute a finite subset of nodes
of the zone graph satisfying the following properties: for every
uncovered node, all its successors are present; for every covered node
$n$, with corresponding covering node node $n'$, we have $n$ is
simulated by $n'$ with respect to $n'.\Gg$; finally if $n \to n'$ is a
transition, then for every $n_1$ such that $n_1 \fleq n$ via $\Gg$, we
have $n'_1 \fleq n'$ via $\Gg'$ where $n_1 \to n'_1$.

\begin{lemma}
If $Z \sqsubseteq_{\scriptscriptstyle {R[\Gg]}} Z'$ then $[R]Z \lug [R]Z'$.
\end{lemma}

\begin{lemma}
Suppose $(q, Z') \xra[R]{g} (q_1, Z'_1)$. Let $\Gg, \Gg_1$ be set of
guards such that
\begin{align*}
  \Gg := \begin{cases}
    R[\Gg_1] \cup g & \text{ if } Z' \not \sqsubseteq_{\scriptscriptstyle
      {R[\Gg_1]}} Z' \cap g \text{ and } \\
    R[\Gg_1] & \text{ otherwise }
    \end{cases}
  \end{align*}
Then for every zone $Z$ s.t. $Z \lug Z'$, the successor $(q, Z)
\xra[R]{g} (q_1, Z_1)$ satisfies $Z_1 \sqsubseteq_{\scriptscriptstyle
  {\Gg_1}} Z'_1$.
\end{lemma}
\begin{proof}
If $\Gg = R[\Gg_1] \cup g$, then the lemma is true with proof same as
in the case of static analysis. Suppose $\Gg = R[\Gg_1]$. This is the
case when $g$ is not considered. By definition, this will imply that
$Z' \sqsubseteq_{\scriptscriptstyle {R[\Gg_1]}} Z' \cap g$.  Now, if $Z
\lug Z'$, then as $\Gg = R[\Gg_1]$ we get $Z
\sqsubseteq_{\scriptscriptstyle {R[\Gg_1]}} Z' \cap g$. Hence $Z \cap
g \sqsubseteq_{\scriptscriptstyle {R[\Gg_1]}} Z' \cap g$, from which
we can derive that $Z_1 \sqsubseteq_{\scriptscriptstyle
      {\Gg_1}} Z'_1$. \qed
  \end{proof}

  \begin{lemma}
 For every $(q, Z)$ reachable in the zone
 graph, there is an uncovered node $(q, Z')$ with a set of guards
 $\Gg'$ such that $Z \lugprime Z'$.
\end{lemma}
\begin{proof}
By induction on the length of the path to $(q, Z)$ from the initial
node. Base case is trivially true, since we explore $(q_0, Z_0)$ in
the dynamic algorithm.

Suppose the lemma is true for $(q,Z)$ with $(q, Z')$ being the
covering node. Consider a successor $(q, Z)
\xra[R]{g} (q_1, Z_1)$ in the zone graph. Since $(q, Z', \Gg')$ is
uncovered, the successor $(q_1, Z_1, \Gg'_1)$ is present. The
propagation step satisfies the conditions given in the above
lemma. If $(q_1, Z'_1)$ is uncovered, this will be the node
corresponding to $(q_1, Z_1)$. If $(q_1, Z'_1, \Gg'_1)$ is covered by
$(q_1, Z''_1, \Gg''_1$ then the propagation ensures that $\Gg'_1
\supseteq \Gg''_1)$. Hence $Z_1 \sqsubseteq_{\scriptscriptstyle
  {\Gg''_1}} Z''_1$, from which we get $(q_1, Z''_1)$ as the required node
for $(q_1, Z_1)$. \qed
  \end{proof}

